Meta-Learning and Universality: Deep Representations and Gradient Descent can Approximate any Learning Algorithm

Learning to learn is a powerful paradigm for enabling models to learn from data more effectively and efficiently. A popular approach to meta-learning is to train a recurrent model to read in a training dataset as input and output the parameters of a learned model, or output predictions for new test inputs. Alternatively, a more recent approach to meta-learning aims to acquire deep representations that can be effectively fine-tuned, via standard gradient descent, to new tasks. In this paper, we consider the meta-learning problem from the perspective of universality, formalizing the notion of learning algorithm approximation and comparing the expressive power of the aforementioned recurrent models to the more recent approaches that embed gradient descent into the meta-learner. In particular, we seek to answer the following question: does deep representation combined with standard gradient descent have sufficient capacity to approximate any learning algorithm? We find that this is indeed true, and further find, in our experiments, that gradient-based meta-learning consistently leads to learning strategies that generalize more widely compared to those represented by recurrent models.

==> experiments_workshops.tex <==
\vspace{-0.1cm}
\section{Experiments}
\vspace{-0.2cm}


Now that we have shown that meta-learners that use standard gradient descent with a sufficiently deep representation can approximate any learning algorithm, we aim to empirically explore the differences between gradient-based and recurrent meta-learners. In particular, we aim to answer the following questions: (1) can a learner trained with MAML further improve from additional gradient steps when learning new tasks at test time, or does it start to overfit? and (2) does the inductive bias of gradient descent enable better few-shot learning performance on tasks outside of the training distribution, compared to learning algorithms represented as recurrent networks?

\begin{figure}[t!]
\setlength{\unitlength}{0.5\columnwidth}
\begin{picture}(1.99,0.4) \linethickness{0.5pt}
\put(0.0,0.0){\includegraphics[height=0.225\columnwidth]{sine_indistr.png}}
\put(0.66,0.0){\includegraphics[height=0.225\columnwidth]{sine_amp.png}}
\put(1.33,0.0){\includegraphics[height=0.225\columnwidth]{sine_phase.png}}
%\put(0.1,-0.05){\includegraphics[width=0.9\columnwidth]{oneshot_diagram_two_heads.pdf}}

\end{picture}
\vspace{-0.2cm}
\caption{\footnotesize The effect of additional gradient steps at test time when attempting to solve new tasks. The MAML model, trained with $5$ inner gradient steps, can further improve with more steps. All methods are provided with the same data -- 5 examples -- where each gradient step is computed using the same 5 datapoints.
\label{fig:gradstep_results} 
\vspace{-0.3cm}
}
\end{figure}



\begin{figure}[t!]
%\vspace{-0.6cm}
\setlength{\unitlength}{0.5\columnwidth}
\begin{picture}(1.99,0.4) \linethickness{0.5pt}
\put(0.0,0.0){\includegraphics[height=0.22\columnwidth]{omni_shear.png}}
\put(0.66,0.0){\includegraphics[height=0.22\columnwidth]{omni_scale.png}}
\put(1.33,0.0){\includegraphics[height=0.22\columnwidth]{sine_amprange.png}}
%\put(0.1,-0.05){\includegraphics[width=0.9\columnwidth]{oneshot_diagram_two_heads.pdf}}

\end{picture}
\vspace{-0.2cm}
\caption{\footnotesize Learning performance on out-of-distribution tasks as a function of the task variability. Recurrent meta-learners such as TCML and MetaNet acquire learning strategies that are less generalizable than those learned with gradient-based meta-learning.
\label{fig:metaextrap} 
\vspace{-0.4cm}
}
\end{figure}

To study both questions, we will consider two simple few-shot learning domains. The first is 5-shot regression on a family of sine curves with varying amplitude and phase. We trained all models on a uniform distribution of tasks with amplitudes $A\in[0.1, 5.0]$, and phases $\gamma \in[0, \pi]$. The second domain is 1-shot character classification using the Omniglot dataset~\citep{omniglot}, following the training protocol introduced by Santoro et al.~\cite{mann}.
In our comparisons to recurrent meta-learners, we will use two state-of-the-art meta-learning models: TCML~\citep{tcml} and meta-networks~\citep{metanetworks}. In some experiments, we will also compare to a task-conditioned model, which is trained to map from both the input and the task description to the label. Like MAML, the task-conditioned model can be fine-tuned on new data using gradient descent, but is not trained for few-shot adaptation. We include more experimental details in Appendix~\ref{app:exps}.

\begin{wrapfigure}{r}{0.36\textwidth}
    \begin{center}
    \vspace{-0.7cm}
        \includegraphics[width=0.36\textwidth]{omni20curve.png}
    \end{center}
    \vspace{-0.4cm}
    \caption{\footnotesize 
    %An initialization learned with MAML can be fine-tuned for 100 gradient descent steps without overfitting.
    Comparison of finetuning from a MAML-initialized network and a network initialized randomly, trained from scratch. Both methods achieve about the same training accuracy. But, MAML also attains good test accuracy, while the network trained from scratch overfits catastrophically to the 20 examples. Interestingly, the MAML-initialized model does not begin to overfit, even though meta-training used 5 steps while the graph shows up to 100.
    %does not begin to overfit with more gradient steps, even though meta-training used only 5 steps, while the graph shows up to 100.
    }
    \vspace{-0.5cm}
    \label{fig:learningcurve}
\end{wrapfigure}

To answer the first question, we fine-tuned a model trained using MAML with many more gradient steps than used during meta-training. The results on the sinusoid domain, shown in Figure~\ref{fig:gradstep_results}, show that a MAML-learned initialization trained for fast adaption in 5 steps can further improve beyond $5$ gradient steps, especially on out-of-distribution tasks. In contrast, a task-conditioned model trained without MAML can easily overfit to out-of-distribution tasks. We also ran this experiment with the Omniglot dataset. As seen in Figure~\ref{fig:learningcurve}, a MAML model that was trained with $5$ inner gradient steps can be fine-tuned for $100$ gradient steps without leading to any drop in test accuracy.
As expected, a model initialized randomly and trained from scratch quickly reaches perfect training accuracy, but overfits massively to the $20$ examples.

Next, we investigate the second question, aiming to compare gradient-based meta-learning with state-of-the-art recurrent meta-learners on a variety of tasks that are related to, but outside of the distribution of training tasks. All three methods achieved similar performance within the distribution of training tasks for 5-way 1-shot Omniglot classification and 5-shot sinusoid regression. In the Omniglot setting, we compare each method's ability to learn to compare digits that have been sheared or scaled by varying amounts. In the sinusoid regression setting, we compare on sinusoids with larger amplitudes in the range $[5.0,10.0]$ and phases in the range $[\pi, 2\pi]$.
The results in Figure~\ref{fig:metaextrap} and Appendix~\ref{app:exps} show a clear trend that MAML recovers more generalizable learning strategies. %, demonstrating an effective inductive bias. 
Combined with the theoretical universality results, these experiments indicate that deep gradient-based meta-learners are not only equivalent in representational power to recurrent meta-learners, but should also be a considered as a strong contender in settings that contain domain shift between meta-training and meta-testing tasks, where their strong inductive bias for reasonable learning strategies provides substantially improved performance.


==> introduction_workshops.tex <==
\section{Introduction}

%\todo{go through intro and problem statement again with Justin's comments in mind -- quantifiers that a sufficiently expressive RNN meta-learner can approximate any learning algorithm when outputting weights of any function class. If the function class is limited, however, then you can't get any function of x,x*, y... which doesn't satisfy our definition of universal learning algorithm approximator.}

Deep neural networks that optimize for effective representations have enjoyed tremendous success over human-engineered representations. 
Meta-learning takes this one step further by optimizing for a learning algorithm that can effectively acquire representations. A common approach to meta-learning is to train a recurrent or memory-augmented model such as a recurrent neural network 
to take a training dataset as input and then output the parameters of a learner model~\citep{schmidhuber1987,bengiobengio1,learntooptimize,learntolearnbygdbygd}. Alternatively, some approaches pass the dataset and test input into the model, which then outputs a corresponding prediction for the test example~\citep{mann,rl2,learningrl,tcml}.
Such recurrent models are \emph{universal learning algorithm approximators}, in that they have the capacity to approximately represent any mapping from dataset to algorithm. However, depending on the form of the model, it may lack statistical efficiency.
%%SL.10.19: maybe elaborate on why it might lack statistical efficiency (larger input space)

In contrast to the aforementioned approaches, more recent work has proposed methods that include the structure of optimization problems into the meta-learner~\citep{hugo,maml,husken}.
In particular, model-agnostic meta-learning (MAML) optimizes \emph{only} for the initial parameters of the learner model, using standard gradient descent as the learner's update rule~\citep{maml}.
Then, at meta-test time, the learner is trained via gradient descent.
By incorporating prior knowledge about gradient-based learning, MAML improves on the statistical efficiency of black-box meta-learners and has successfully been applied to a range of meta-learning problems~\citep{maml,mil,li2017learning}.
But, does it do so at a cost? A natural question that arises with purely gradient-based meta-learners such as MAML is whether it is indeed sufficient to only learn an initialization, or whether representational power is in fact lost from not learning the update rule. Intuitively, we might surmise that learning an update rule is more expressive than simply learning an initialization for gradient descent.
In this paper, we seek to answer the following question: does simply learning the initial parameters of a deep neural network have the same representational power as arbitrarily expressive meta-learners that directly ingest the training data at meta-test time? Or, more concisely, does representation combined with standard gradient descent have sufficient capacity to constitute any learning algorithm?
%%CF: Alternative phrasing for above: "is representation enough to constitute any learning algorithm"
%%CF: I'm calling it a learning algorithm to suggest that the algorithm is conditioned on training data.

In this paper, we analyze this question from the standpoint of the universal function approximation theorem. We compare the theoretical representational capacity of the two meta-learning approaches: a deep network updated with one gradient step, and a meta-learner that directly ingests a training set and test input and outputs predictions for that test input (e.g. using a recurrent neural network).
In studying the universality of MAML, we find that there exists a form of learner model for which MAML has the same theoretical representational power as recurrent meta-learners. 
We therefore conclude that, when using deep, expressive function approximators, there is no theoretical disadvantage in terms of representational power to using MAML over a black-box meta-learner represented, for example, by a recurrent network.

%Our analysis of the universality of MAML involves analyzing the form of the gradient during weight updates. This analysis also suggests that the expressivity of the MAML update can be substantially improved by a small architectural modification that does not alter the representational power of the network, but does increase the representational power of the gradient. %Our empirical evaluation confirms that this architectural modification leads to substantially improved performance in terms of both meta-learning speed and generalization.

Since MAML has the same representational power as any other universal meta-learner, the next question we might ask is: what is the benefit of using MAML over any other approach? We study this question by analyzing the effect of continuing optimization on MAML performance.
Although MAML optimizes a network's parameters for maximal performance after a fixed small number of gradient steps, we analyze the effect of taking substantially more gradient steps at meta-test time.
%Since MAML optimizes a network's parameters with the aim of enabling it to improve as much as possible from a fixed, small number of gradient steps, we might wonder
%%SL.10.19: a little much wondering (we are wondering in the above sentence, and in the sentence before that)
% fixed.
%whether taking more gradient steps further improves performance, and whether it might lead to more overfitting when training at meta-test time on very small training sets. 
We find that initializations learned by MAML are extremely resilient to overfitting to tiny datasets, in stark contrast to more conventional network initialization, even when taking many more gradient steps than were used during meta-training.
We also find that the MAML initialization is substantially better suited for extrapolation beyond the distribution of tasks seen at meta-training time, when compared to meta-learning methods based on networks that ingest the entire training set. We analyze this setting empirically and provide some intuition to explain this effect.
%%SL.10.19: great intro! now we just have to make sure the paper lives up to this!



==> problem_statement_workshop.tex <==

\vspace{-0.1cm}
\section{Problem Statement}
\vspace{-0.25cm}

%Our goal is to compare the flexibility of the recurrent model meta-learning approach to that of learning a representation and running gradient descent (MAML).
%%SL.10.24: could omit the above sentence (also not clear if that is indeed our goal -- we want to show universality)

We can broadly classify RNN-based meta-learning methods into two categories.
In the first approach~\citep{mann,rl2,learningrl,tcml}, there is a meta-learner model $\rnn$ with parameters $\phi$ which takes as input the dataset $\dataset_\task$ for a particular task $\task$ and a new test input $\testinp$, and outputs the estimated output $\testout$ for that input:
$$
\testout = \rnn(\dataset_\task, \testinp ; \phi) = \rnn((\inp, \out)_1, ..., (\inp, \out)_K, \testinp ; \phi)
%\testout = \rnn(\dataset_\task, \testinp ; \phi) = \rnn(\{(\inp, \out)_k\}, \testinp ; \phi)
$$
The meta-learner $g$ is typically a recurrent model that iterates over the dataset $\dataset$ and the new input $\testinp$.
For a recurrent neural network model that satisfies the UFA theorem, this approach is maximally expressive, as it can represent any function on the dataset $\dataset_\task$ and test input $\testinp$.

In the second approach~\citep{hochreiter,bengiobengio1,learntooptimizenn,learntolearnbygdbygd,hugo,hypernets}, there is a meta-learner $\rnn$ that takes as input the dataset for a particular task $\dataset_\task$ and the current weights $\theta$ of a learner model $f$, and outputs new parameters $\theta_\task'$ for the learner model.
Then, the test input $\testinp$ is fed into the learner model 
to produce the predicted output $\testout$.
The process can be written as follows:
$$
%\testout = f (\testinp ; \theta_\task') = f(\testinp; \rnn(\dataset_\task; \phi)) = f(\testinp; \rnn(\{(\inp, \out)_k\} ; \phi))\\
\testout = f (\testinp ; \theta_\task') = f(\testinp; \rnn(\dataset_\task; \phi)) = f(\testinp; \rnn((\inp, \out)_{1:K} ; \phi))
$$
Note that, in the form written above, this approach can be as expressive as the previous approach, since the meta-learner could simply copy the dataset into some of the predicted weights, reducing to a model that takes as input the dataset and the test example.\footnote{For this to be possible, the model $f$ must be a neural network with at least two hidden layers, since the dataset can be copied into the first layer of weights and the predicted output must be a universal function approximator of both the dataset and the test input.}
Several versions of this approach, i.e.~\cite{hugo, learntooptimizenn}, have the recurrent meta-learner operate on order-invariant features such as the gradient and objective value averaged over the datapoints in the dataset, rather than operating on the individual datapoints themselves.
%%CF: TODO need to check the references here to make sure that they actually do this.
%define the function $\rnn$ as an average over the datapoints in the dataset:
%$$
%\rnn(\{(\inp, \out)_i\} ; \phi) = \frac 1N \sum_i \tilde{\rnn} ((\inp, \out)_i ; \phi)
%$$
This induces a potentially helpful inductive bias that disallows coupling between datapoints, ignoring the ordering within the dataset. As a result, the meta-learning process can only produce permutation-invariant functions of the dataset.
%That said, this setting becomes more expressive if the meta-learner is allowed to update the learner weights more than once in SGD settings. In particular, it can learn any function of the dataset and its ordering in $K$ steps of SGD with minibatches of size 1. We will discuss the expressivity of performing multiple updates in Section~\ref{sec:kshot}.


In model-agnostic meta-learning (MAML), instead of using an RNN to update the weights of the learner $f$, standard gradient descent is used. Specifically, the prediction $\testout$ for a test input $\testinp$ is:
$$
\testout = f_{\text{}} (\testinp ; \theta_\task') = f_{\text{}} (\testinp ; \theta - \alpha \nabla_\theta \loss(\dataset_\task, \theta)) 
= f_{\text{}} \left(\testinp ; \theta - \alpha \nabla_\theta \frac 1K \sum_{k=1}^K   \loss(\out_k, f_{\text{}}(\inp_k;\theta))\right),
$$
where $\theta$ denotes the initial parameters of the model $f$ and also corresponds to the parameters that are meta-learned. 
Since the RNN approaches can approximate any update rule, they are clearly at least as expressive as gradient descent.
It is less obvious whether or not the MAML update imposes any constraints on the set of update functions that can be learned.


The first goal of this paper is to show that $f_{\text{MAML}} (\testinp ; \theta_\task')$ is a universal function approximator of $(\dataset_\task, \testinp)$
in the one-shot setting, where the dataset $\dataset_\task$ consists of a single datapoint $(\inp,\out)$.
Then, we will consider the case of $K$-shot learning, showing that $f_{\text{MAML}} (\testinp ; \theta_\task')$ is universal in the set of functions that are invariant to the permutation of datapoints. In both cases, we will discuss meta supervised
learning problems with both discrete and continuous labels and the loss functions under which universality does or does not hold. %Finally, we will discuss learning functions that are \emph{not} invariant to the dataset ordering using meta-learned loss functions.
%\todo{delete last sentence if we decide not to include meta-learned loss functions.}

%We will consider settings where the loss function 
%An outline of the proof is as follows: First, we will show that the $\frac{d\loss}{d\act_i}$ can be any continuous function of the error derivative $\frac{d\loss}{d f_\theta(\dataset_\task)}$. Then, we will discuss scenarios in which the error derivative can be a universal function approximator of the input and/or label in the dataset. Finally, we will show that, under certain architectural assumptions, the weight matrices and biases can be any function of the dataset. \todo{See previous todo about how this statement isn't correct.}
